Gaussian Plane-Wave Neural Operator for Electron Density Estimation

This work studies machine learning for electron density prediction, which is fundamental for understanding chemical systems and density functional theory (DFT) simulations. To this end, we introduce the Gaussian plane-wave neural operator (GPWNO), which operates in the infinite-dimensional functional space using the plane-wave and Gaussian-type orbital bases, widely recognized in the context of DFT. In particular, both high- and low-frequency components of the density can be effectively represented due to the complementary nature of the two bases. Extensive experiments on QM9, MD, and material project datasets demonstrate GPWNO's superior performance over ten baselines.

==> 4_method_old.tex <==


\section{Preliminary}

% \textbf{Molecular graph and crystal graph.}  We are interested in learning the map from the geometric graph  to the continuous function over the euclidean space. We use the $\gM=(\gX,\gA)$ to denote the molecular graph and $\rho_\gM:\sR^3 \to \sR$ to denote the continuous function. Specifically, $n$ atoms molecular can be represented by the its atomic positions $\gX=[\vx_1,\ldots,\vx_n]^\top \in \sR^{3\times n}$ and atomic features $\gA=[\va_1,\ldots,\va_n]^\top\in \sR^{d_a\times n}$. In addtion, some molecular system like crystal can be represented by the its periodic pattern to form infinitely large molecular. In the periodic case, we use the unit cell representation $\gM=(\gX, \gA, \gL)$ with the unit cell lattice $\gL =[\vl_1,\vl_2,\vl_3]^\top \in \R^{3\times 3}$ and original (infintely large) molecular is represented by $\gM_\infty =(\gX_\infty,\gA_\infty)$ where
% \begin{align*}
%     \gX_\infty&=\{\hat \vx_{\vk,i}|\hat \vx_{\vk,i} = \vx_i+\sum^{3}_{j=1}k_j\vl_j, \vk\in \mathbb \mathbb{Z}^{3},i\in N\}\\
%     \gA_\infty&=\{\hat \va_{\vk,i}|\hat \va_{\vk,i}=\va_i,\vk\in \mathbb \mathbb{Z}^{3},i\in N\}
% \end{align*}
% with $N = \{1,\ldots,n\}$ and $\vk=(k_1,k_2,k_3) \in \mathbb \mathbb{Z}^{3}$. Consequently, $X_\infty$ contains all possible translation of $X$ as amounts of integer multiples of $L$ and $P_\infty$ is its atomic features. Our main idea is the molecular $M=(X,A)$ and crystal $\tilde M=(X,A,L)$ whose lattice is large enough $(\|l_i\| >c)$ maps to the similar continuous function $\rho_M \approx \rho_{\tilde M}$. Thus, we build the methods from the periodical graph and generalize it to the general molecular graph

\textbf{Periodic and aperiodic molecular graph.}   Our focus is learning the mapping from geometric graphs to continuous functions over Euclidean space. We represent an (aperiodic) molecular graph as $\gM=(\gX,\gA)$ and the corresponding continuous function as $\rho_\gM:\sR^3 \to \sR$.  Specifically, a molecular structure with $n$ atoms is denoted by atomic positions $\gX=[\vx_1,\ldots,\vx_n]^\top \in \sR^{3\times n}$ and atomic features $\gA=[\va_1,\ldots,\va_n]^\top\in \sR^{d_a\times n}$. For periodic structures, such as crystals, we represent them using their periodic patterns, forming an infinitely large molecular graph. In these cases, we employ the unit cell representation $\tilde \gM=(\gX, \gA, \gL)$, with the unit cell lattice $\gL =[\vl_1,\vl_2,\vl_3]^\top \in \R^{3\times 3}$. The original infinite molecular structure is then given by $\gM_\infty =(\gX_\infty,\gA_\infty)$, where
\begin{align*}
    \gX_\infty&=\left\{\hat \vx_{\vk,i}\bigg\vert\hat \vx_{\vk,i} = \vx_i+\sum^{3}_{j=1}k_j\vl_j, \vk\in \mathbb \mathbb{Z}^{3},i\in \mN\right\},\\
    \gA_\infty&=\left\{\hat \va_{\vk,i}|\hat \va_{\vk,i}=\va_i,\vk\in \mathbb \mathbb{Z}^{3},i\in \mN\right\}
\end{align*}
with $\mN = \{1,\ldots,n\}$ and $\vk=(k_1,k_2,k_3) \in \mathbb \mathbb{Z}^{3}$. Consequently, $X_\infty$ encompasses all possible translations of $X$ by integer multiples of $L$, and $A_\infty$ represents its atomic features. Our hypothesis posits that a molecular structure $\gM=(\gX,\gA)$ and a crystal $\tilde \gM=(\gX,\gA,\gL)$, with sufficiently large lattice vectors ($|l_i| >c$), map to similar continuous functions $\rho_M \approx \rho_{\tilde \gM}$. This forms the foundation of our method, initially developed for periodic graphs and extended to general molecular graphs.

% In addtion, some molecular system like crystal can be represented by the its periodic pattern to form infinitely large molecular. In the periodic case, we use the unit cell representation $\gM=(\gX, \gA, \gL)$ with the unit cell lattice $\gL =[\vl_1,\vl_2,\vl_3]^\top \in \R^{3\times 3}$ and its original (infintely large) molecular is represented by $\gM_\infty =(\gX_\infty,\gA_\infty)$ where
% \begin{align*}
%     \gX_\infty&=\left\{\hat \vx_{\vk,i}|\hat \vx_{\vk,i} = \vx_i+\sum^{3}_{j=1}k_j\vl_j, \vk\in \mathbb \mathbb{Z}^{3},i\in N\right\},\\
%     \gA_\infty&=\left\{\hat \va_{\vk,i}|\hat \va_{\vk,i}=\va_i,\vk\in \mathbb \mathbb{Z}^{3},i\in N\right\}
% \end{align*}
% with $N = \{1,\ldots,n\}$ and $\vk=(k_1,k_2,k_3) \in \mathbb \mathbb{Z}^{3}$. Consequently, $X_\infty$ contains all possible translations of $X$ as amounts of integer multiples of $L$ and $A_\infty$ is its atomic features. Our main idea builds on the assumption that molecular $M=(X,A)$ and crystal $\tilde M=(X,A,L)$ whose lattice is large enough $(\|l_i\| >c)$ maps to the similar continuous function $\rho_M \approx \rho_{\tilde M}$. Thus, we build the methods from the periodical graph and generalize it to the general molecular graph.


% https://nwchemgit.github.io/pw-lecture.pdf
\textbf{Plane-wave basis.} The plane-wave basis is a flexible basis widely used in the electronic structure calculations of solid-state systems \cite{martin_2004}. In any periodic system confined within lattice $\gL$, we can represent the system using the plane-wave basis set. Formally, the discrete translation of lattice vectors
$$\mathbf R_\vn = n_1\vl_1 + n_2\vl_2 +n_3\vl_3,\text{where } \vn =(n_1,n_2,n_3) \in \mathbb{Z}^{3}$$
allows to find the corresponding wavevector $$\mathbf G_\vm = m_1\vb_1 + m_2\vb_2 +m_3\vb_3,\text{where } \vm =(m_1,m_2,m_3) \in \mathbb{Z}^{3}   $$ satisfying $$\mathbf G_\vm\cdot\mathbf R_\vn = 2\pi N \text{, where } N \in \mathbb Z.$$


% Any periodic system that is bounded by the lattice $\gL$ can be represented by the plane-wave basis set. Formally, the discrete translation of the lattice vector
% $$\mathbf R_\vn = n_1\vl_1 + n_2\vl_2 +n_3\vl_3,\text{where } \vn =(n_1,n_2,n_3) \in \mathbb{Z}^{3}$$
% can always find the wavevector $$\mathbf G_\vm = m_1\vb_1 + m_2\vb_2 +m_3\vb_3,\text{where } \vm =(m_1,m_2,m_3) \in \mathbb{Z}^{3}   $$ that satisfies $$\mathbf G_\vm\cdot\mathbf R_\vk = 2\pi N \text{ where } N \in \mathbb Z.$$

These wavevectors $\mathbf G_\vm$ are constructed from reciprocal primitive vectors $(\vb_1,\vb_2,\vb_3)$ satisfying $\vl_i\cdot\vb_j=2\pi\delta_{ij}$:
\begin{align*}
\vb_i = \frac{2\pi}{V} \vl_j \times \vl_k
\end{align*}
where $V=\vl_i\cdot(\vl_j\times\vl_k)$ and $(ijk)=(123)$\footnote{$(i,j,k)\in\{(1,2,3),(2,3,1),(3,1,2)\}$}.

% Those wavevectors $\mathbf G_\vm$ are formed by the reciprocal primitive vectors $(\vb_1,\vb_2,\vb_3)$ satisfies $\vl_i\cdot\vb_j=2\pi\delta_{ij}$:
% \begin{align*}
%     \vb_i = \frac{2\pi}{V} \vl_j \times \vl_k
% \end{align*}
% where $V=\vl_i\cdot(\vl_j\times\vl_k)$ and $(ijk)=(123)$.

Any continuous function $u(\vx)$ follows the lattice periodicity and translating $\vx$ by any lattice vector $\mathbf R_\vn$ yields the same value:
\begin{equation*}
u(\vx) = u(\vx+ \mathbf R_\vn).
\end{equation*}
Expressing this function in terms of the plane-wave basis, we obtain
\begin{equation*}
u(\vx)=\sum_{\vm} \hat u_\vm \exp (i\mathbf G_\vm \cdot \vx).
\end{equation*}
and this expression naturally satisfies the periodicity. With the orthogonality and completeness of the plane-wave basis, any periodic bounded function $\rho$ can be represented this way.

% Any continuous function $u(\vx)$ follows the periodicity of the lattice, translating $\vx$ by any lattice vector $\mathbf R_\vn$ poses the same value:
% \begin{equation*}
%     u(\vx) = f(\vx+ \mathbf R_\vn).
% \end{equation*}

% Expressing the above function in terms of the plane-wave basis, we have
% \begin{equation*}
%     u(\vx)=\sum_{\vm} \hat u_\vm \exp (i\mathbf G_\vm \cdot \vr).
% \end{equation*}

% Since the plane-wave basis is orthogonal and complete, we can express any periodic bounded $\rho$ in principle.

However, this becomes impractical when dealing with deep learning due to the necessity of a large number of basis functions. The 3D Euclidean functions need 3D Fourier basis which requires $O(L^3)$ space complexity along the system size $L$.


% But this is possible when there exists large numbers of the basis. But this is inapplicable when you dealing it with the deep learning.

\textbf{Localized Gaussian-type orbital based basis.} Gaussian-type orbitals (GTO) offer an alternative basis set for expressing electronic structures. The Gaussian basis functions follow a radial-angular decomposition:
$$\psi_{nlm}(\vr) = R^l_n(r)Y^m_l(\hat \vr)=c_{nl}\exp(-a_nr^2)r^lY^m_l(\hat \vr)$$
where $Y^m_l(\hat \vr)$ represents spherical harmonics and $r=\|\vr\|$ is the vector length, and $\hat \vr=\vr/r$ is the direction of the vector on the unit sphere. The degree $l$ of spherical harmonics is a non-negative integer and the magnetic order $m$ is an integer satisfying $-l \le m \le l$.

Employing a multicentric expansion scheme, we can also express $\rho_{\gM}$ using the GTO basis functions:
\begin{equation*}
    \rho_{\gM}(\vr) = \sum^n_{i=1}\sum_{nlm} f^i_{nlm}\psi_{nlm}(\vr-\vx_i),
\end{equation*}
where $f^i_{nlm}$ are the basis coefficients of $\psi_{nlm}$ and $\vx_i$ is its atomic position for $i$-th atom.

Recent research incorporates GTO basis with deep neural network-based coefficient learning \citet{cheng2023equivariant}. {\color{mydarkblue}However, GTO-based methods face limitations, particularly in addressing long-range regions from atom centers and maintaining periodic boundary conditions, due to exponential convergence in corner cases.}

% Recently, there exist some researches that incorporate the GTO basis with the coefficient learning with the deep neural networks. However, GTO-based approaches pose some limitations in that it is converge exponentially at the corner case so it is hard to address the long-range regions form the atom centers, also hard to retain the periodic bound conditions.

% \textbf{Pseudo Potential}
% blah blah

\section{Method}

We decompose the target function $\rho(\vx)$ into high-frequency dominating and low-frequency dominating functions with respect to the plane-wave-basis sets:
\begin{equation*}
    \rho(\vx) = \rho_{\text{high}}(\vx) + \rho_{\text{low}}(\vx)
\end{equation*}

We hypothesize that the short-ranged regions from the atom centers necessitate high-frequency plane-wave bases, whereas the long-ranged regions require low frequencies. Intuitively, we replace the high-frequency region with the GTO-based basis and leverage the plane-wave basis in low-frequency region.

% We hypothesize the short-ranged part needs high frequencies plane-wave basis but the long-ranged part needs low frequencies. Thus, we try to predict the short-range regions with the GTO-based basis and the long-ranged regions with the plane-wave basis.

\textbf{GTO based coefficient learning.} Our approach for the high-frequency regions utilizes GTO-based coefficient learning derived from the \citet{cheng2023equivariant} framework. The outputs of the $\rho_{\text{high}}$ is
\begin{equation*}
    \rho_{\text{high}}(\vx) = \sum_{nlm} f_{nlm} \psi_{nlm}(\vx)
\end{equation*}
where the $f_{nlm}$ is updated by the message passing
\begin{align}
    \mathbf f^{nl}_u &\leftarrow \sum_{v\in \gN(u)} \sum_{k\le 0} W^{nlk}(\vx_{v}-\vx_u)\mathbf f^{nk}_v, \\
    W^{nlk}(\vr)  &= \sum^{k+1}_{J=\|k-l\|}\varphi^{lk}_J(r) \sum^J_{m=-J} Y^m_J(\hat \vr) Q^{lk}_{Jm}.
\end{align}
Herein, $Q^{lk}_{Jm}$ is the Clebsh-Gordan matrix of shape $(2l+2)\times(2k+1)$ and $\varphi^{lk}_J: \mathbb R^+ \to \mathbb R$ are learnable radial net.


\textbf{Plane-wave basis expansion.}  To maintain the periodic boundary condition $\rho(\vx) = \rho(\vx+ \mathbf R_\vn)$, we employ the Fourier transform with the plane-wave basis set in the sense of the wavevector $G$ and lattice $\gL$. Detailed explanations are placed in the appendix. Main intuition is started from the fact that any arbitrary vector x can be expressed by the lattice coordinate framework:
\begin{equation*}
\vx = z_1\vl_1 + z_2 \vl_2 + z_3 \vl_3 = \vz,
\end{equation*}

where $z_1,z_2,z_3 \in \mathbb R$.

From the above lattice coordinate, we can define new function $\rho_\gL$:
\begin{equation*}
     \rho_{\gL}\left(z_1,z_2,z_3\right)= \rho\left(z_1\vl_1 + z_2 \vl_2 + z_3 \vl_3\right)
\end{equation*}
or we can write it as $\rho_{\gL}(\vz) = \rho_{\gL}\left(z_1,z_2,z_3\right)$.

% \rho_{\gL}(z_1,z_2,z_3)  = \rho(\vx)
% To initiate, we express any arbitrary vector $\vx$ within the lattice coordinate framework:

% \footnote{Note that $K(\vr)=K(\vr+\mathbf R_\vn)$ should be satisfied to maintain the periodic boundary conditions}

% To satisfy the periodic boundary condition, we use the Fourier transform along with the plane-wave basis set.
%  transform of a function, in the sense of the wavevector $G$ First, we can write any arbitrary $\vx$ in the coordinate system of the lattice:
% \begin{equation*}
% \vx = z_1\vl_1 + z_2 \vl_2 + z_3 \vl_3 = \vz,
% \end{equation*}

% where $z_1,z_2,z_3 \in \mathbb R$.

% And we can define new function $\rho_{\gL}$:
% \begin{equation*}
%     \rho_{\gL}(z_1,z_2,z_3)  = \rho(\vx) = \rho\left(z_1\vl_1 + z_2 \vl_2 + z_3 \vl_3\right)
% \end{equation*}

This $\rho_{\gL}(\vz)$ is now a function of three variables, each of which has periodicity 1, respectively.
% \begin{equation*}
%     \rho_{\gL}(z_1,z_2,z_3) = \rho_{\gL}(z_1+n_1,z_2+n_2,z_3+n_3)
% \end{equation*}
% where $n_1,n_2,n_3 \in \mathbb Z$.
Then, we can easily compute the Fourier series expansions of $\rho_{\gL}$ with the reciprocal basis $\vm = m_1\vb_1 + m_2\vb_2 + m_3\vb_3$:
\begin{equation}
\begin{aligned}
\rho_{\gL}(\vz)=\sum_{\vm\in \mathbb \mathbb{Z}^{3}} \hat\rho_{\gL}(\vm)
\cdot\exp\left(i2\pi\left(\vm \cdot \vz \right)\right),
\end{aligned}
\end{equation}


where $\hat\rho_{\gL}(\vm) = \int^1_0 dz_3 \int^1_0 dz_2 \int^1_0 dz_1 \rho_{\gL}(\vz)\exp\left(-2i\pi\left(\vm\cdot\vz\right)\right)$.


Using the definition $\vl_i\cdot \vb_j = 2\pi \delta_{ij}$, we can substitute $\vm\cdot\vz$:
\begin{align*}
    \mathbf G_\vm \cdot \vz  &=2\pi (m_1 z_1 + m_2 z_2 + m_3z_3) = 2\pi \vm\cdot\vz,
\end{align*}
where naturally $\mathbf G_\vm \cdot \vz = \mathbf G_\vm \cdot \vx$ is satisfied by definition.
    % \vm\cdot\vz &= m_1z_1 + m_2z_2 +m_3z_3, \\

% \begin{align*}
%     \mathbf G_\vm \cdot \vz &= (m_1 \vb_1 + m_2\vb_2 + m_3 \vb_3)\cdot(z_1 \vl_1 + z_2 \vl_2 + z_3 \vl_3)\\
%     & =2\pi (m_1 z_1 + m_2 z_2 + m_3z_3)
% \end{align*}

Eventually, it is clear that
\begin{equation}
    \rho(\vx)=\sum_{\vm\in \mathcal \mathbb{Z}^{3}} \hat \rho_{\gL}(\vm ) \exp (i\mathbf G_\vm \cdot \vx).
    \label{eq:plane_wave_expanion}
\end{equation}

% \begin{equation}
%     \hat\rho_\theta(\vm) = \mathcal F^{-1}(R_\phi)
% \end{equation}


\textbf{Reciprocal Neural Oeprator.}
% What we try to learn is the $\rho(\vx)$, and in the view of the coefficient learning, we will try to learn the $\hat \rho_\gL(\vm)$. Since the $\rho_\gL(\vm)$ is the W

We used the Discrete Fourier Transformation to bulid the plane-wave basis expansion in \eqref{eq:plane_wave_expanion}.  The outputs of the $\rho_{\text{low}}$ are learned iterative in the reciprocal space.

First, initialize the $\rho^{(0)}$ based on the interpolation network. To leverage the FFT algorithms, we located the uniformly voxelized probe points set $P$ as the $n\times n \times n$ in 3D lattice. That is $\|P\|=n^3$ and $\vx_p = (k_1,k_2,k_3)$ where $k_1,k_2,k_3 \in \{0,1/n,\ldots,(n-1)/1\}$.

For given any prove points $p \in \gP$ at coordinate $\vx_p$, we aggregated messages from the atoms nears probe points $p$: 
\begin{equation}
   \rho^{(0)}(\vx_p) = \sum_{v \in \tilde \gN(\gA;p)}\frac{1}{\|\tilde \gN(\gA;p)\|}h_\theta(\|\vx_p-\vx_v\|,\va_v),
\end{equation}
where $\tilde \gN(\gA;p)$ is the set of the periodical neighbor list in $\gA$ from probe node $p$. And change the $\rho^{(0)}$ to $\rho^{(0)}_{\gL}$ by change of the basis.

Let's assume that $\tilde \gF$ is a discrete Fourier transform, then we can also use the direct parameterized kernel $R_\phi$ in the Reciprocal space using the convolution theorem \citep{li2021fourier}:
\begin{equation}
    \rho_{\gL}^{(t+1)}(\vz)=\left(\gK \rho_{\gL}^{(t)}\right)(\vz) = \tilde{\gF}^{-1}\left(R_\phi \cdot \left(\tilde{\gF} \rho_{\gL}^{(t)}\right) \right) (\vz)
\end{equation}
where $R_\phi$ is the Fourier transform of a kernel function $K$ and the detailed proofs are in the appendix.




% Afterwards, we can define the kernel integral method transformation parameterized by a neural network
% ,
% \begin{equation*}
%     (\gT_w \rho^{(t)}_{lr})(\vx) = \int_{\mathbb R^3} K_\phi(\vx-\vy) \rho^{(t)}_{lr}(\vy) \text{d}\vy.
%     \label{eq:kernel_integral}
% \end{equation*}

% We can also use the direct parameterized kernel $R_\phi$ in the Reciprocal space using the convolution theorem  \citep{li2021fourier}:
% \begin{equation*}
%     (\gK \rho_{\gL})(\vz) = \gF^{-1}\left(R_\phi \cdot (\gF \rho_{\gL}) \right)
% \end{equation*}
% where $R_\phi$ is the Fourier transform of a kernel function $K$ in \eqref{eq:kernel_integral}.




% We used the traditional neural operator-based learning scheme. The outputs of the $\rho_{\text{low}}$ are learned iterative in the reciprocal space. So we will parameterize the plane-wave basis coefficient $\hat \rho_{\gL}$ in \eqref{eq:plane_wave_expanion}.
% \begin{equation}
%     \hat\rho_{\gL}(\theta;\vm) = (\gF \rho_\gL)(\vm) \cdot R_\theta (\vm)
% \end{equation}
% in the reciprocal space.

% \begin{align}
%     \hat\rho_{\gL}(\theta;\vm) = (\gF \rho_\gL)(\vm)\\
%     \\ = \int 
% \end{align}
% where $\gF$ is the Fourier transform.

% Afterwards, we can define the kernel integral method transformation parameterized by a neural network
% ,
% \begin{equation*}
%     (\gT_w \rho^{(t)}_{lr})(\vx) = \int_{\mathbb R^3} K_\phi(\vx-\vy) \rho^{(t)}_{lr}(\vy) \text{d}\vy.
%     \label{eq:kernel_integral}
% \end{equation*}


% For given any prove points $p$ at coordinate $\vx$, we aggregated messages from the atoms nears points $p$: 
% \begin{equation*}
%    \rho^{(0)}_{\text{low}}(\vx) = \sum_{v \in \gN(p)}\frac{1}{\|\gN(p)\|}h_\theta(\|\vx-\vx_v\|,\va_v).
% \end{equation*}

% Afterwards, we can define the kernel integral method transformation parameterized by a neural network
% ,
% \begin{equation*}
%     (\gT_w \rho^{(t)}_{lr})(\vx) = \int_{\mathbb R^3} K_\phi(\vx-\vy) \rho^{(t)}_{lr}(\vy) \text{d}\vy
%     \label{eq:kernel_integral}
% \end{equation*}

% Using the relation in the above equation, we use the Fourier transform on the lattice system coordinate $\vz$:
% \begin{align}
%     (\gF \rho_{\gL})(\vm) = \int_D \rho_{\gL}(\vz)\exp(-i2\pi\vm \cdot \vz)\text{d}\vz \\
%     (\gF^{-1} \hat\rho_{\gL})(\vz) = \int_D \hat\rho_{\gL}(\vm)\exp(i2\pi\vm \cdot\vz)\text{d}\vm.
% \end{align}

% We can also use the parameterized kernel $R_\phi$ in the Reciprocal space using the convolution theorem  \citep{li2021fourier}:
% \begin{equation*}
%     (\gK \rho_{\gL})(\vz) = \gF^{-1}\left(R_\phi \cdot (\gF \rho_{\gL}) \right)
% \end{equation*}
% where $R_\phi$ is the Fourier transform of a periodic kernel function $K$ in \eqref{eq:kernel_integral}.

% This implies learning parametized $\rho_\theta(\vm)$:
% \begin{equation}
%     \hat\rho_\theta(\vm) = (R_\phi \cdot \gF\rho_\gL)(\vm)
% \end{equation}

After iterative updating of the lattice coordinate systems of function $\rho^{(t)}_{\gL}(\vz)$,  we change the basis to the Euclidean
\begin{equation}
    \rho^{(T)}(\vx) = \rho^{(T)}_{\gL}(\vz).
\end{equation}

% (Fix it to the voxelized grid) But actually, above $\rho_{\text{sr}}$ is finite voxelized points in the space

Consequently, $\rho^{(T)}$ is voxelized value in the space, we can interpolate the values in the space by usign query node to get the arbitrary features in the space:
\begin{equation}
    \rho_{\text{low}}(\vx) = \sum_{p \in \tilde \gN(\gP;\vx)} \frac{1}{\|\tilde \gN(\gP;\vx)\|}f_\theta(\|\vx-\vx_p\|,\rho^{(t)}(\vx_p)),
\end{equation}
where $\tilde \gN(\gP;\vx)$ is the set of the periodical neighbor list in $\gP$ from the coordinate $\vx$.

\textbf{Masking the high-frequency regions}

Motivated by the logic of the density functional, we simply masked the region near the atom, and our results is
\begin{equation*}
    a(\vx) = 
    \begin{cases} 1 \quad\text{if } d(\vx,\vy) > c_{\text{mask}}, \quad \forall \vy \in \gA \\
    0 \quad \text{else}.
    \end{cases}
\end{equation*}

Integrated all, our method predicts the continuous function by
\begin{equation*}
    \hat \rho(\vx) = \rho_{\text{high}}(\vx) + a(\vx)\rho_{\text{low}}(\vx)
\end{equation*}


% Expressing the above function in terms of the plane-wave basis, we have
% \begin{equation*}
%     u(\vx)=\sum_{\vm} \hat u_\vm \exp (i\mathbf G_\vm \cdot \vr).
% \end{equation*}
% In addition, we use the Reciprocal integral operator which is the Fourier Neural Operator in Reciprocal,
% \begin{equation*}
%     (
% \end{equation*}



% Intuitively, what we are doing is finding long-range signal from the given molecular system.

% We started it in the periodical case and notice that electronic density function or charge density fucntion of the periodical system like crystal should be written in the plane wave basis function. The plane wave basis function is the spatial Fourier basis whose frequency is reciprocal of cell length. In short, principly, we should express the electronic density function of crystal by the Fourier basis.

% But, unfortunately, the result of \cite{cheng23} shows that FNO which uses the convolution operation in the Fourier space is not suitable to use it directly to this problem. So we focused on not only use the spherical harmonics but also Fourier

% I assume that there exists there are two parts of the function - short range from the atoms where spherical harmonics can express well and long range where fourier basis can express well.

% So in the sense of the convolution.
% Let $\gG=(\gA,\gF)$ is the atomic graph and $a\in\gA\subset \sR^3$ is the set of positions of atom, $f\in\gF\subset \sR^d$ is the atom features, 

% \begin{equation*}
%     F: \gG \mapsto \rho
% \end{equation*}
% \begin{equation*}
%     [F(\gG)](\mathbf x) = \rho_{\gG}(\mathbf x)
% \end{equation*}

% Let $h(\mathbf y) = \sum_{\mathbf a \in \gA} \delta^3(\mathbf y - \mathbf a)$

% \begin{equation*}
%     F(\gG,\gA) = \int_D W(\mathbf x, \mathbf y) h(\mathbf y)
% \end{equation*}
% \begin{equation*}
%     \rho(\mathbf r) = \rho_{\text{sr}}(\mathbf r) + \rho_{\text{lr}}(\mathbf r)
% \end{equation*}

% \begin{align}
%     \gT \rho(x) &:= \int_D W(\mathbf x,\mathbf y) \rho(\mathbf y) d \mathbf y \\
%     &= \sum_{u \in \gV}\sum^\infty_{i=1}f_{i,u}\psi_i(\mathbf x - \mathbf r_u).
% \end{align}

% Kernel formulation

% \begin{equation*}
%     A(\mathbf x) = \int_D k(x,y, a(x),a(y)) h(y)dy
% \end{equation*}

% \subsection{Coefficient Learning}

% \subsection{Reciprocal Neural Operator}

% \subsection{Pseudo Potential}

==> 5_experiment_old.tex <==
\section{Experiment}

\subsection{Baselines and evaluation metrics}
To evaluatethe models, we followed \citet{jorgensen2020deepdft} and \citet{cheng2023equivariant} and use the definition of the \textit{normalized mean absolute error} (NMAE) as our evaluation metrics:
\begin{equation}
    \text{NMAE} = \frac{\int_\R^3 \|\hat\rho(\vx)-\rho(\vx)\|\text{d}\vx}{\int_\R^3 \|\rho(\vx)\|\text{d}\vx}
\end{equation}

Although we trained from the sampled grid from the full voxel, We did the full evaluation on the partitioned mini-batches of the full density grid.

\input{Tables/1_main_table}
\subsection{Density prediction for aperiodic systems}
\textbf{QM9} The QM9 dataset \citep{ruddigkeit2012enumeration, ramakrishnan2014quantum} contains 133,884 small molecule species consisting  C,H,O,N and F. The QM9 electron charge density dataset and its data splits built by \citep{Jørgensen_Bhowmik_2022} which gives 123,835 training samples, 50 validation samples and 10,000 test samples.

% The QM9 dataset contains 133885 small molecules consisting of C, H, O, N, and F. The QM9 electron density dataset was built by Jørgensen et al. (paper) and was publicly available via Figshare. Each tarball needs to be extracted, but the inner lz4 compression should be kept. We provided code to read the compressed lz4 file.



\textbf{Cubic}
We conducted thorough experiments on extensive electron density datasets, and showed that our RNO models has the state-of-the-art performance compared to existing baselines. Additionally, we performed several ablation studies to highlight the efficacy of our proposed architecture.


% The Cubic dataset contains electron charge density for 16421 (after filtering) cubic crystal system cells. The dataset was built by Wang et al. (paper) and was publicly available via Figshare. Each tarball needs to be extracted, but the inner xz compression should be kept. We provided code to read the compressed xz file.
The Cubic dataset \citep{wang2022large} contains electron charge density for 17,418 cubical lattice inorganic material. We use the same filtration and data splits in \citet{cheng2023equivariant}. The remaining data points are 16,421 and the data splits are 14,421, 1,000 and 1,000 for train/validation/test was pre-assigned. 

% This large-scale dataset contains electron densities on 17,418 cubic inorganic materials [53].
% In our experiment setting, we first filtered out the noble gas (He, Ne, Ar, Kr, Xe) and kept only the
% crystal structure whose primitive cell contains less than 64 atoms. This gave 16,421 remaining data
% points. A data split of 14421, 1000, and 1000 for train/validation/test was pre-assigned.

\textbf{MD} The MD dataset 6 small molecules ethanol, benzene, phenol, resorcinol, ethane, malonaldehyde with different positions sampled from molecular dynamics (MD). The dataset was curated by \citep{bogojeski2018efficient,bogojeski2020quantum}. The former 4 molecules has 1000 train sampled geometry and 500 test, the latter has 2000 and 400 respectively. The model were independently trained  for each molecule.

\textbf{Results.} 
In \cref{tab:main1}, one can observe how our algorithm outperforms the existing baselines by a large margin. 

 % triclinic, monoclinic, orthorhombic, tetragonal, trigonal, hexagonal, and cubic.
\subsection{Density prediction for periodic systems}
\textbf{Dataset.} The Materials Project (MP) \citep{jain2013commentary} contains the inorganic materials and its properties. We used the electronic charge density property of 120,775 molecule built by \citet{shen2021representationindependent}. We filtered the broken files and categorized by 7 different lattice system (triclinic, monoclinic, orthorhombic, tetragonal, trigonal, hexagonal,cubic) and 1 mixed dataset of former 7 dataset. Each dataset has 7,681 to 26,081 train samples and 1,000 or 500 validation and test splits are pre-assigned. The detailed train configurations in the appendix.

\input{Tables/2_sub_mp}

\input{Tables/3_ablation_methods}


% https://home.iitk.ac.in/~sangals/crystosim/crystaltut.html
\subsection{Ablation study}


\textbf{Pseudo Potential and RNO}


==> Figures/conceptual.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/conceptual5.pdf}
    \caption{\textbf{Overview of our method.} Starting from the input molecule with its atomic positions, atomic features, and lattice vectors, our task aims to predict the electron density $\rho_{\text{pred}}$ of input molecular at the given query points in continuous space. Notably, our approach decomposes this prediction into two components: GTO-based and PW-based. The GTO-based layer directly predicts the coefficients of the GTO basis and, subsequently, $\rho_{\text{GTO}}$ is determined by multiplying these coefficients with the expanded basis. PW-based layer introduces probe nodes, which are uniformly distributed within the lattice. Each probe node aggregates the message from nearby atoms to predict the low-frequency representations of the PW basis. As a result, the PW layer predicts $\rho_{\text{PW}}$ by aggregating the messages from neighboring probe nodes relative to the query node}    \label{fig:method}
\end{figure*}

    % \captionsetup{justification=raggedright,
    % singlelinecheck=false
    % }
    % $\rho_{\text{pred}}(\cdot)\in \R$ for given query point $\vx_q \in \gQ$ in continuous space. Notably, we decompose the prediction into two parts: \textbf{GTO based} and \textbf{PW based}. (upper) GTO based layer adapted equivariant message passing scheme with node-wise spherical features. The layer predicts the coefficients of the GTO basis and predict $\rho_{\text{GTO}}(\vx_q)$ by combining the multiplication of the expanded basis and coefficients. (lower) PW based layer present the virtual probe nodes $\vx_p \in \gP$ which are uniformly spaced inside the $\mL$ and each node aggregates the message from the near atoms. Then, predict the low-frequency representations of the PW basis. Finally, predict $\rho_{\text{PW}}$ at $\vx_q$ by aggregating the messages from the neighbor probe nodes $N_\gP$ of the query node $\vx_q$.}

==> Figures/fig_visualization_app.tex <==


% \newcommand{\addpic}{\includegraphics[width=6em]{example-image}}
% \newcommand{\addpicv}[1]{\includegraphics[trim={1.35cm 1.35cm 1.35cm 1.35cm},clip,width=4.2em]{#1}}
% \newcommand{\addpicqm}[1]{\includegraphics[trim={2.7cm 2.7cm 2.7cm, 2.2cm},clip,width=4.2em]{#1}}
% \newcommand{\addpich}[1]{\includegraphics[trim={2.1cm 2.1cm 2.1cm 2.1cm},clip,width=4.2em]{#1}}

\newcolumntype{C}{>{\centering\arraybackslash}m{4.2em}}
\begin{figure*}
\centering
\setlength\tabcolsep{1pt} % default value: 6pt
% \setlength\tabrowsep{1pt} % default value: 6pt
\begin{tabular}{l*9{C}@{}}
\toprule
Name & \multicolumn{3}{c}{QM9} & \multicolumn{3}{c}{Tetragonal} & \multicolumn{3}{c}{Hexagonal} \\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}& GT & GPW-NO & InfGCN & GT & GPW-NO & InfGCN & GT & GPW-NO & InfGCN \\ 
\midrule

& \addpicqm{output_figure/qm9/GPW_6_target.png}  
& \addpicqm{output_figure/qm9/GPW_6_diff2.png}
& \addpicqm{output_figure/qm9/infgcn_6_diff2.png}
& \addpicv{output_figure/tetragonal/GPW_0_target.png}  
& \addpicv{output_figure/tetragonal/GPW_0_diff.png}
& \addpicv{output_figure/tetragonal/infgcn_0_diff.png}
& \addpich{output_figure/hexagonal/GPW_0_target.png}  
& \addpich{output_figure/hexagonal/GPW_0_diff.png}
& \addpich{output_figure/hexagonal/infgcn_0_diff.png}\\ 
\midrule
NMAE(\%) &~&0.47&0.59&~&5.48&5.78 &~&9.26&9.69\\
\bottomrule 
\end{tabular}
\caption{caption}
\label{fig:vis_app}
\end{figure*} 

% https://tex.stackexchange.com/questions/310807/how-to-generate-a-table-of-figures

==> Tables/4_inference.tex <==
 \begin{table}[h!]
    \centering
    \begin{tabular}{lcc}
    \toprule
    Model / dataset & MD (benzene) & MP (mixed) \\
    \midrule
    DeepDFT & 1  & 3\\
    DeepDFT2 & 1  & 3\\
    InfGCN & 1 & 3\\
    \textbf{Ours} & 1  & 3\\
    \bottomrule 
    \end{tabular}
    \caption{Inference time (s) for each models}
    \label{tab:inference}
\end{table}


==> algorithm/gto.tex <==
\begin{algorithm}[tb]
   \caption{Gaussian type orbital-based prediction}
   \label{alg:pw}
\begin{algorithmic}[1]
   \STATE \textbf{Input:} Molecular system $\mathcal{M}=(\mathcal{X}, \mathcal{A}, \mathbf{L})$
   \STATE Sample $t\sim \text{Uniform}(1,\ldots,T)$
   \STATE Sample $\bm{y}^{(t)}\sim q(\bm{y}^{(t)}|\bm{y}^{(0)})$
   \STATE Compute $\mu_{\theta}(\bm{y}^{(t)})$ and $\hat{\mu}$
   \STATE Update $\theta$ to minimize $\frac{1}{\sigma^{2}_{t}}\| \bm{\mu}_{\bm{\theta}}(\bm{y}^{(t)})-\hat{\bm{\mu}}\|^{2}_{2}$
\end{algorithmic}
\end{algorithm}


==> algorithm/pw.tex <==
\begin{algorithm}[tb]
   \caption{Plane wave-based prediction}
   \label{alg:pw}
\begin{algorithmic}[1]
   \STATE \textbf{Input:} Molecular system $\mathcal{M}=(\mathcal{X}, \mathcal{A}, \mathbf{L})$, voxelized density function $\gV$, number of the query points $K$
   \STATE Randomly sample the $K$ query points $P$ from $\gV$
   \STATE Update the atomic features
   \STATE $\mK \leftarrow $
   \STATE Sample $t\sim \text{Uniform}(1,\ldots,T)$
   \STATE Sample $\bm{y}^{(t)}\sim q(\bm{y}^{(t)}|\bm{y}^{(0)})$
   \STATE Compute $\mu_{\theta}(\bm{y}^{(t)})$ and $\hat{\mu}$
   \STATE Update $\theta$ to minimize $\frac{1}{\sigma^{2}_{t}}\| \bm{\mu}_{\bm{\theta}}(\bm{y}^{(t)})-\hat{\bm{\mu}}\|^{2}_{2}$
\end{algorithmic}
\end{algorithm}

